Inferring Drop-in Binary Parsers from Program Executions

We present BIEBER (Byte-IdEntical Binary parsER), the first system to model and regenerate a full working parser from instrumented program executions. To achieve this, BIEBER exploits the regularity (e.g., header fields and array-like data structures) that is commonly found in file formats. Key generalization steps derive strided loops that parse input file data and rewrite concrete loop bounds with expressions over input file header bytes. These steps enable BIEBER to generalize parses of specific input files to obtain parsers that operate over input files of arbitrary size. BIEBER also incrementally and efficiently infers a decision tree that reads file header bytes to route input files of different types to inferred parsers of the appropriate type. The inferred parsers and decision tree are expressed in an IR; separate backends (C and Perl in our prototype) can translate the IR into the same language as the original program (for a safer drop-in replacement), or automatically port to a different language. An empirical evaluation shows that BIEBER can successfully regenerate parsers for six file formats (waveform audio [1654 files], MT76x0 .BIN firmware containers [5 files], OS/2 1.x bitmap images [9 files], Windows 3.x bitmaps [9971 files], Windows 95/NT4 bitmaps [133 files], and Windows 98/2000 bitmaps [859 files]), correctly parsing 100% (>= 99.98% when using standard held-out cross-validation) of the corresponding corpora. The regenerated parsers contain automatically inserted safety checks that eliminate common classes of errors such as memory errors. We find that BIEBER can help reverse-engineer file formats, because it automatically identifies predicates for the decision tree that relate to key semantics of the file format. We also discuss how BIEBER helped us detect and fix two new bugs in stb_image as well as independently rediscover and fix a known bug.

==> evaluation-arxiv.tex <==


\section{Evaluation}
\label{sec:evaluation}

We implemented \slime and used it to empirically evaluate the effectiveness of the \slime pipeline. We evaluate \slime using the BMP (bitmap image) and WAV/WAVE (waveform audio) file formats. BMP and WAV are classic, eponymous file formats for bitmap images and waveform audio files.~\cite{bmp4_spec,bmp5_spec,wave_format}   They are still in wide use today, some 30 or so years after they were first
introduced (with a number of revisions over the years).




\elcheaposubsection{Bitmap Parser}
\label{sec:evaluation_bmp}

\noindent\textbf{Image Corpus.} Our corpus contains 11,008 unique 16/24/32-bit bitmap files. %
Files range in size from 6,966 bytes (48x48 24-bit) to 36,578,358
bytes (3024x4023 24-bit), with a total corpus size of 16,283,146,489 bytes.

We built the corpus by obtaining the top 10 most popular search phrases for each of the 25 English-text categories from Google's
Year in Search 2018 \cite{google_yis_2018}.
We then used \code{google\_images\_download} \cite{google_images_download} to scrape the top 100 bitmap images from Google Image Search for
each of the 232 unique keywords.
This returned a median of 68 bitmaps per phrase (min 1, max 92) due to various errors
(\eg ``Wrong image format returned''), for a total of 13,694 bitmaps.

We filtered out: corrupted bitmaps (contains less pixel data than implied by the dimensions; 168 files),
duplicate (byte-for-byte identical) copies of bitmaps (1980 files),
files that are not ``PC bitmap'' (1 GIF and 3 JPEG), palettized bitmaps (448 files)
and 32-bit bitmaps with all-zero alpha channels (86 files).


\noindent\textbf{Effectiveness of pipeline.} We applied the \slime pipeline to the entire corpus.
The generated parser decision tree (Figure \ref{fig:stb_image_parse_tree}) is a complete binary tree with 20 leaves (each leaf corresponds to a parser for a specific input file format) that correctly parses all 11,008 bitmaps (\ie 100\% correctness).

At each node, we show the predicate from its parent; for example, the root is split based on whether byte 28 of the file --- the bit-depth of the image --- is 24.
We list, at each node, the number of bitmaps that can be successfully parsed using the best-available individual parser, if the node's subtrees were pruned. The leaves show our description of each parser's functionality; for example, the right-most leaf parses 16-bit (5-6-5\footnote{\ie 5 bits for blue, 6 bits for green, 5 bits for red}) bottom-up bitmaps.


The full tree spans
many variations of bitmaps, such as bottom-up \vs top-down, OS/2 \vs Windows, and different subpixel
arrangements (BGRA, RGBA, ARGB for 32-bit;
5-6-5 and 5-5-5 for 16-bit).




\begin{figure}
\centering
\includegraphics[scale=0.6]{figures/ParseTree_catimg_final1001_Copy669_truncated_vertical.pdf}
\caption{
\textbf{Generated parser decision tree for \stbimage's BMP functionality.}}
\label{fig:stb_image_parse_tree}
\end{figure}


\noindent\textbf{Training/test performance.} To evaluate the generalizability of our automatically generated parser, we performed standard
held-out cross-validation~\cite{isl}. We randomly split 80\% of our corpus into a training set
(8806 bitmaps), ran the complete \slime pipeline, and then tested on the
remaining held-out 20\%. We repeated this process a total of 100 times
to account for the random split.
Our pruned decision trees correctly parsed between 99.93\% and 100.00\% of
the entire corpus (average 99.98\%). The parsing failures occur when
rare bitmap classes are represented in the test set but not the training set.

We note that the original parser correctly parses only $\approx 98\%$ of the
corpus, because it contains bugs which \slime helped us find and fix and which our regenerated parser avoids.

\elcheaposubsection{Waveform Audio Parser}
\label{sec:casestudy_WAV}

Our audio corpus contains 70 \code{.wav} audio files. These files differ based on the number of channels (i.e., mono vs. stereo), sampling rate, and recording length. The mapping from input file to in-memory data structures can be non-trivial; for stereo audio files, the input is interleaved channels, each containing 16-bit \code{short}s, while the output is separate (left- and right- channel) arrays of 64-bit \code{long}s.

Our generated decision tree, trained on the ten smallest audio files, includes parsers for both mono and stereo formats and  successfully parses all 70 files in the corpus.








\elcheaposubsection{Relevant Predicates}
\label{sec:deconstruct_file_format}

The parser decision tree (Figure \ref{fig:stb_image_parse_tree}), as a whole, is useful for parsing the entire corpus of bitmaps. However, it is also notable that, for each of the internal nodes, Algorithm \ref{algo:pick-a-choose} has automatically chosen predicates that are meaningful for the file format, \textit{without} using the BMP file specification, nor any explicit control-flow information from the original parser (recall that the \diode logs do not contain such information). We discuss some of the predicates that \slime has chosen.

As noted earlier, the first decision in the tree, \code{in[28] == 24}, tests if the bit-depth of the image is 24. The predicate \code{in[10] == 138} checks the offset of the pixel data in the file, or equivalently, the size of the header and therefore the version of the bitmap file format. Another internal node identifies whether an image is top-down (\code{height < 0}) or bottom-up (\code{height > 0}). Our predicate selection (Algorithm~\ref{algo:pick-a-choose}) can only test strict equality of individual bytes, yet it is able to determine if the height field is negative by taking advantage of the two's complement representation of 32-bit integers (\code{in[24] == 0}). Additionally, although our predicate selection algorithm can only test single bytes, it chooses the correct parser for different 4-byte bitmasks by recursively partitioning on individual bytes until they are disambiguated, in a similar fashion to Blind ROP's byte-by-byte discovery of stack canaries~\cite{bittau2014hacking}. Unlike Blind ROP's hardcoded strategy, this byte-by-byte discovery is an emergent property of \slime's decision tree algorithm.





\elcheaposubsection{Memory safety enhancements}
\label{sec:memory_safety}

Our code examples use direct array accesses \eg \code{out [0] = in
[70]}. Our actual implementation uses a wrapper function to prevent reading
past the bounds of the input file, and replaces the output array
with a dynamic array to prevent any buffer overflows or underflows. These
enhancements are enabled in our code generation backend. They do not require
any developer input, changes to the original parser, or identification of any such bugs.

\elcheaposubsection{Finding other bugs (\emph{not} related to memory safety)}
\label{sec:bug_finding}
During our development and testing of \slime, we found and reported two new bugs in the
\stbimage library.
We also independently rediscovered an old bug. Notably, neither of the new bugs lead to memory-safety
issues, and therefore would not have been avoided by (re-)writing \stbimage in a memory-safe
language or running \stbimage with a memory error detector such as AddressSanitizer~\cite{address_sanitizer}.

\noindent\textbf{New bug \#1: missing bytes.}\footnote{\url{https://github.com/nothings/stb/issues/773}} For 16-bit bitmaps with
compression type 3 (user-specified red/green/blue
bitmasks), \stbimage skipped the first 12 bytes of the pixel data, because
it did not account for the bitmasks when seeking from the end of the header to the start of the pixel data.
We were
able to identify this bug --- \textit{without} comparing \stbimage to a second parser ---
because the \diode logs for these
bitmaps were also missing the first 12 bytes, which made loop abstraction
impossible. %
The \stbimage maintainer noted the bug report and fixed it in a subsequent release.





\noindent\textbf{New bug \#2: irrelevant bitmask.}\footnote{\url{ https://github.com/nothings/stb/issues/783}} For 32-bit bitmaps with
compression type 0 (no bitmasks), the user-specified
color channel bitmasks should be ignored according to the
specification~\cite{bmp4_spec,bmp5_spec}. \stbimage correctly checks the
compression field for Windows 3.x bitmaps, but for Windows 95/98/2000 bitmaps,
it always uses the bitmasks.
For the vast majority of Windows 95/98/2000 32-bit bitmaps, this does not result
in a bug, because the color channel bitmasks contain values equivalent to
the default (BGRA). However, for $\approx 1\%$ of our corpus, this has a
visible discrepancy, because the bitmask specifies RGBA. Our tree partitioning
algorithm grouped these images into their
own ``RGBA-parser'' leaf, making it easy to identify this class of bug-triggering
inputs by inspection.



\noindent\textbf{Old bug \#1: irrelevant bitmask redux.} For 24-bit bitmaps where the
``alpha mask'' header field is non-zero, \stbimage outputs a \emph{32-bit} (RGBA) image with the alpha channel set to 255 (fully opaque). Although the input and output images are visually identical, this is not the desired API behavior (as shown by the maintainer having fixed this bug), unnecessarily increases memory usage by one-third, and could cause a buffer overflow if the library user had only allocated enough for memory for a 24-bit image and blindly copied \stbimage's bloated output.
We identified this bug because our tree partitioning algorithm grouped the bug-triggering inputs (all but one of the
24-bit Windows 98 bitmaps) into their own leaf.
This bug has some overlap with our New bug 2; however, the fix for this bug (as of \stbimage 2.25) is highly specific
to 24-bit bitmaps and does not address the new bugs.




\noindent\textbf{Classes of detectable bugs.}
\slime, by design, cannot automatically confirm that a behavior is buggy; strange behaviors can be deliberate ``features,'' and \slime's decision tree will faithfully replicate them. It does, however, assist with triaging the test cases for manual review, as files with the same behavior/bug will often be handled by the same leaf parser.

\slime can help detect bugs that manifest in buggy images being parsed by separate, buggy parser(s) (\eg in our new bug \#2, there was a leaf for Windows 95/98/2000 32-bit bitmaps with an RGBA bitmask). Conceptually, the decision tree has extra leaves for the buggy inputs, where, by some unusual criterion, the buggy inputs are separated from regular inputs. Debugging is simplified because we have both the test case, \emph{and} the criteria that distinguishes buggy \vs non-buggy inputs.

We can also quickly test the parser decision tree by inspecting the parser's output for one bitmap corresponding to each of the leaves. If the bug-triggering inputs are underrepresented in the corpus --- likely the case, as the bug would otherwise have already been discovered through ordinary testing --- then inspecting each leaf parser (with one test case each) is much more efficient than randomly sampling input files. The bug-triggering bitmaps for the two new bugs we identified are rare (each $\approx 1\%$ of our bitmap corpus),
highlighting both the coverage of our corpus and \slime's sensitivity to bugs.

Two special subclasses of detectable bugs are parsers that violate our high-level model of parsed data structures (that data is hyperrectangular, with dimensions defined by header fields; see new bug \#1) and buffer overflows (old bug \#1 may lead to this in application code, under some circumstances). These two subclasses result in parsing behavior that is so peculiar that they can often be manually confirmed as bugs, without comparing the output to another parser.

\slime does not efficiently detect bugs that manifest in buggy images being parsed by an inappropriate, but preexisting parser (\ie if the bug has resulted in merged or switched leaves/parsers in the decision tree). However, if these bugs result in buffer overflows, \slime will still prevent them by construction in the regenerated parser (as discussed earlier), even if we could not detect them in the original parser.

\elcheaposubsection{Optimized processing}

The bitmap parser results required eight iterations of
\textsc{ExpandLogsUntilConverged} (Algorithm \ref{algo:active-learning-diode}),
with \diode logs for only 74 of the 11,008 BMPs.
Figure \ref{fig:active_learning} shows the number of unparseable BMPs (across all leaves of the parser decision tree) at the start of each
round. At the start of round 0, the entire corpus (11,008 BMPs, totaling 16GB) cannot be parsed. The 10 smallest BMPs total just 132KB; after processing these smallest BMPs, only 1,809 bitmaps ($< 18\%$ of the corpus by file count or size) are unparseable.
We then repeat the process by selecting the 10 next smallest unparseable BMPs (328KB), until converged. In total, we ran \diode on just 12.8MB of BMPs (0.08\% of the corpus by file size).

\noindent\textbf{Comparison with other file selection strategies.}
We measured the amount of time required for \code{dfsan\_parse} to process \diode logs 
for selected BMP and WAV files, then used these measurements to build performance models that characterize the time required to obtain the final \slime parser (the vast majority of this time is spent in \code{dfsan\_parse}). With these models, the time required to process a BMP file is
$0.0692B$ seconds; the time to process a WAV file is $0.2157B$, where $B$ is the number of bytes in the BMP or WAV file. 


Table \ref{fig:log_strategies} uses these models to compare the number of bytes of input needed to be run through the instrumented parser, and corresponding approximate CPU days required, for various file selection strategies.

In the absence of Algorithm \ref{algo:active-learning-diode} --- which used the insight that we can test whether inputs are already parseable by our regenerated parsers --- we would need to generate \diode logs for all the files and feed them into Algorithm \ref{algo:tree-learning}. For the bitmap corpus, this would be prohibitively expensive: roughly 13,000 CPU days. This is orders of magnitude slower than Algorithm \ref{algo:active-learning-diode}, which only requires around 10 CPU days. We do have some extra overhead from rebuilding the tree and testing the parsers, but this
is negligible compared to \diode's runtime.

 

We also model the runtime of Algorithm \ref{algo:active-learning-diode} with a different heuristic than choosing the smallest unparseable files at each round. When choosing the \textit{largest} unparseable files, the modeled runtime is 500 CPU days; this is still much faster than running \diode on all the logs, but also significantly slower than choosing the smallest files. We also tried random selection: the runtimes were in between (35 or 85 days). 

The WAV results are less exaggerated but follow the same general pattern, again showing that Algorithm \ref{algo:active-learning-diode} with our smallest size heuristic provides a significant speedup.




\begin{figure}
\resizebox{1.0\columnwidth}{!}{
\begin{tabular}{ | c | r | r | r | r }
\hline
& \multicolumn{3}{c|}{Unparseable bitmaps} \\
\hline
Round & \makecell{\# files} & \makecell{\# bytes (all)} & \makecell{\# bytes (10 smallest)} \\
\hline
0 & 11,008 & 16,283,146,489 &  131,492 \\
1 &  1,809 &  2,913,068,807 &  328,480 \\
2 &  1,260 &  2,059,278,713 &  591,480 \\
3 &  1,085 &  1,913,469,901 &  871,512 \\
4 &    308 &    736,009,768 & 1,247,716 \\
5 &    106 &    284,912,770 & 1,733,040 \\
6 &     58 &    191,820,812 & 3,890,752 \\
7 &      4 &      3,992,704 & 3,992,704 \\
8 &      0 &              0 &         0 \\
\hline
TOTAL &    &                & 12,787,176 \\
\hline
\end{tabular}
}
\caption{
\textbf{
Number of unparseable bitmaps (across all leaves)
at different algorithm iterations.
}
Round 0 is the initial corpus of 11,008 bitmaps. At each round, we generate \diode logs for the 10 smallest unparseable bitmaps, and then re-run
\code{BuildTree} (Algorithm \ref{algo:tree-learning}).
}
\label{fig:active_learning}
\end{figure}



\begin{figure*}
\centering
\begin{tabular}{ | c | r | r | r | r | }
\hline
& \multicolumn{2}{c|}{\textbf{BMP}} & \multicolumn{2}{c|}{\textbf{WAV}} \\
\hline
\textbf{Strategy} & \textbf{Bytes of input} & \textbf{Approx. CPU Days} & \textbf{Bytes of input} & \textbf{Approx. CPU Days} \\
\hline
Process all files & 16,283,146,489 & 13,041.6 & 19,633,150 & 49.0 \\
\hline
Smallest size first & 9,388,502 & 7.5 & 440,546 & 1.1 \\
Largest size first & 621,022,028 & 497.4 & 7,642,682 & 19.1 \\
Random (seed 1) & 107,180,204 & 85.8 & 2,828,230 & 7.1 \\
Random (seed 2) & 43,694,466 & 35.0 & 2,548,802 & 6.4 \\
\hline
\end{tabular}
\caption{
\textbf{
Comparison of file selection strategies, based on our performance model.
}
}
\label{fig:log_strategies}
\end{figure*}











